Who Responded to Whom: The Joint Effects of Latent Topics and Discourse in Conversation Structure

Numerous online conversations are produced on a daily basis, resulting in a pressing need to conversation understanding. As a basis to structure a discussion, we identify the responding relations in the conversation discourse, which link response utterances to their initiations. To figure out who responded to whom, here we explore how the consistency of topic contents and dependency of discourse roles indicate such interactions, whereas most prior work ignore the effects of latent factors underlying word occurrences. We propose a model to learn latent topics and discourse in word distributions, and predict pairwise initiation-response links via exploiting topic consistency and discourse dependency. Experimental results on both English and Chinese conversations show that our model significantly outperforms the previous state of the arts, such as 79 vs. 73 MRR on Chinese customer service dialogues. We further probe into our outputs and shed light on how topics and discourse indicate conversational user interactions.

==> figures/question-answer-example.tex <==
\begin{figure}[h]
% \setlength{\abovecaptionskip}{-0.03cm} 
% \setlength{\belowcaptionskip}{-0.3cm} 
\centering
  \includegraphics[width=\columnwidth ]{ppp.pdf}
%   \vspace{-1em}
    \caption{ \label{fig22}A Wangwang dialogue between a customer (on the left) and a seller (from the server team on the right) from~\citet{he:2019}. Pairwise questions and answers are linked and displayed with the same color.}
\vspace{-2em}
\end{figure}

==> figures/quote-reply-example.tex <==
\begin{figure}[h]
% \setlength{\belowcaptionskip}{-0.3cm} 
% \setlength{\abovecaptionskip}{-0.03cm}
% \setlength{\belowcaptionskip}{-0.cm}
\small 
\begin{tabular}{|p{0.45\textwidth}|}
\hline 
%\multicolumn{1}{p{0.45 \textwidth}}{
\underline{\textbf{Original Post from an Opinion Holder:}}\\  ... Strong family values in society lead to great results. \textit{I want society to take positive aspects of the early Americans and implement that into society.} This would be a huge improvement than what we have now. ...
%}
\\
% \hline 
%\multicolumn{1}{p{0.45 \textwidth}}{
\underline{\textbf{Comment from a Challenger:}}\\ \textit{\&gt; I want society to take positive aspects of the early Americans and implement that into society.} What do you believe those aspects to be? ...
%}
\\
\hline
\end{tabular}
\vspace{-0.5em}
\caption{\label{figure00}An original post and its comment from the \textit{CMV} subreddit. The comment quotes an utterance from the original post (in italic), followed by its reply utterance.
}
\vspace{-2em}
\end{figure}
